3HANDS Dataset: Learning from Humans for Generating Naturalistic Handovers with Supernumerary Robotic Limbs

Supernumerary robotic limbs (SRLs) are robotic structures integrated closely with the user's body, which augment human physical capabilities and necessitate seamless, naturalistic human-machine interaction. For effective assistance in physical tasks, enabling SRLs to hand over objects to humans is crucial. Yet, designing heuristic-based policies for robots is time-consuming, difficult to generalize across tasks, and results in less human-like motion. When trained with proper datasets, generative models are powerful alternatives for creating naturalistic handover motions. We introduce 3HANDS, a novel dataset of object handover interactions between a participant performing a daily activity and another participant enacting a hip-mounted SRL in a naturalistic manner. 3HANDS captures the unique characteristics of SRL interactions: operating in intimate personal space with asymmetric object origins, implicit motion synchronization, and the user's engagement in a primary task during the handover. To demonstrate the effectiveness of our dataset, we present three models: one that generates naturalistic handover trajectories, another that determines the appropriate handover endpoints, and a third that predicts the moment to initiate a handover. In a user study (N=10), we compare the handover interaction performed with our method compared to a baseline. The findings show that our method was perceived as significantly more natural, less physically demanding, and more comfortable.

==> ACMprocess-metadata.tex <==
\title{3HANDS Dataset:\\ Learning from Humans for Generating Naturalistic Handovers with Supernumerary Robotic Limbs}

\author{Artin Saberpour Abadian}
\orcid{0000-0002-5915-5280}
\affiliation{\institution{Saarland University \\ Saarland Informatics Campus}
\city{Saarbr\"{u}cken}
\country{Germany}}
\email{saberpour@cs.uni-saarland.de}

\author{Yi-Chi Liao}
\orcid{0000-0002-2670-8328}
\affiliation{\institution{ETH Z\"{u}rich}
\city{Z\"{u}rich}
\country{Switzerland}}
\email{yichi.liao@inf.ethz.ch}

\author{Ata Otaran}
\orcid{0000-0002-1848-2621}
\affiliation{\institution{Saarland University \\ Saarland Informatics Campus}
\city{Saarbr\"{u}cken}
\country{Germany}}
\email{otaran@cs.uni-saarland.de}

\author{Rishabh Dabral}
\orcid{0009-0004-1245-4146}
\affiliation{\institution{Max Planck Institute for Informatics}
\city{Saarbr\"{u}cken}
\country{Germany}}
\affiliation{\institution{Saarland University \\ Saarland Informatics Campus}
\city{Saarbr\"{u}cken}
\country{Germany}}
\email{rdabral@mpi-inf.mpg.de}

\author{Marie Muehlhaus}
\orcid{0000-0002-5696-7259}
\affiliation{\institution{Saarland University \\ Saarland Informatics Campus}
\city{Saarbr\"{u}cken}
\country{Germany}}
\email{muehlhaus@cs.uni-saarland.de}

\author{Christian Theobalt}
\orcid{0000-0001-6104-6625}
\affiliation{\institution{Max Planck Institute for Informatics}
\city{Saarbr\"{u}cken}
\country{Germany}}
\affiliation{\institution{Saarland University \\ Saarland Informatics Campus}
\city{Saarbr\"{u}cken}
\country{Germany}}
\email{theobalt@mpi-inf.mpg.de}

\author{Martin Schmitz}
\orcid{0000-0002-7332-3287}
\affiliation{\institution{Saarland University \\ Saarland Informatics Campus}
\city{Saarbr\"{u}cken}
\country{Germany}}
\email{mschmitz@cs.uni-saarland.de}

\author{J\"{u}rgen Steimle}
\orcid{0000-0003-3493-8745}
\affiliation{\institution{Saarland University \\ Saarland Informatics Campus}
\city{Saarbr\"{u}cken}
\country{Germany}}
\email{steimle@cs.uni-saarland.de}

==> Source_files/Chapters/Analysis.tex <==
\begin{figure*}[htbp]
    \centering
    % First Row
    \subfloat[participants]{
        \includegraphics[width=0.15\textwidth]{Source/Source_files/Figures/user_direction_1.png}
        \includegraphics[width=0.15\textwidth]{Source/Source_files/Figures/traj_velocity/ID_velocity.png}
    }\label{fig:Participants}
    \hfill
    \subfloat[Primary task type]{
        \includegraphics[width=0.15\textwidth]{Source/Source_files/Figures/traj_analysis/task_type.png}
        \includegraphics[width=0.15\textwidth]{Source/Source_files/Figures/traj_velocity/task_type_velocity.png}
    }\label{fig:prime_task_type}
    \hfill
    \subfloat[Hand-in vs take-away]{
        \includegraphics[width=0.15\textwidth]{Source/Source_files/Figures/traj_analysis/context.png}
        \includegraphics[width=0.15\textwidth]{Source/Source_files/Figures/traj_velocity/context_velocity.png}\label{fig:hand_in vs take_away}
    }
    \\
    % Second Row
    \subfloat[Primary task range]{
        \includegraphics[width=0.15\textwidth]{Source/Source_files/Figures/traj_analysis/prime_range.png}
        \includegraphics[width=0.15\textwidth]{Source/Source_files/Figures/traj_velocity/prime_range_velocity.png}
    }\label{fig:prime_range}
    \hfill
    \subfloat[Primary task height]{
        \includegraphics[width=0.15\textwidth]{Source/Source_files/Figures/traj_analysis/prime_height.png}
        \includegraphics[width=0.15\textwidth]{Source/Source_files/Figures/traj_velocity/prime_height_velocity.png}
    }\label{fig:prime_height}
    \hfill
    \subfloat[Primary task distance]{
        \includegraphics[width=0.15\textwidth]{Source/Source_files/Figures/traj_analysis/prime_distance.png}
        \includegraphics[width=0.15\textwidth]{Source/Source_files/Figures/traj_velocity/prime_distance_velocity.png}
    }\label{fig:prime_distance}
    \caption{Main caption for all figures \textcolor{red}{This would change to a 2D visualizations of interesting properties velocity patterns/ trajectory distributions}}
    \label{fig:combined_images}
\end{figure*}


%=======================================================
\begin{comment}
\begin{figure*}[t] % Place at the top of the page
    \centering
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Source/Source_files/Figures/traj_analysis/ID.png}
        \caption{participants}\label{fig:participants}
    \end{minipage}\hfill
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Source/Source_files/Figures/traj_analysis/task_type.png}
        \caption{prime task type}\label{fig:prime_task_type}
    \end{minipage}\hfill
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Source/Source_files/Figures/traj_analysis/context.png}
        \caption{hand-in vs. take-away}\label{fig:hand_in vs take_away}
    \end{minipage}
     \vspace{10pt} % Add some space between the rows

    % Second row
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Source/Source_files/Figures/traj_analysis/prime_range.png}
        \caption{primary task range}\label{fig:prime_range}
    \end{minipage}\hfill
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Source/Source_files/Figures/traj_analysis/prime_height.png}
        \caption{parimary task height}\label{fig:prime_height}
    \end{minipage}\hfill
    \begin{minipage}{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Source/Source_files/Figures/traj_analysis/prime_distance.png}
        \caption{primary task distance from user body}\label{fig:prime_distance}
    \end{minipage}
\end{figure*}
\end{comment}
\section{Analysis of collected data - will be removed and integrated in Section 3.6}
Out of 936 (780 for now) handovers 370 handover happened between the user's left hand and the WRL and 410 handovers between the user's right hand the WRL. 
\subsection{Trajectories and velocity profiles}
In this section we explore the wrl participants' trajectories based on the parameterization of the user-wrl design space and analyze the findings.  
%
The trajectories are resampled to equal number of samples of 100. 
%
We have evaluated the trajectory similarities using five distinct similarity metrics (see table  \ref{table:similarity-criteria}), across the values of each parameter in our design space.
%
Here is a brief explanation of what each of these similarity metrics mean:
\textbf{Euclidean Distance:} Measures the straight-line distance between two points in multidimensional space.\\
\textbf{DTW (Dynamic Time Warping) Distance:} Measures the similarity between two time series by aligning them to account for shifts and distortions in time.\\
\textbf{Cosine Similarity:} Calculates the cosine of the angle between two vectors, measuring how similar they are in terms of direction rather than magnitude.\\
\textbf{Curve Length Difference:} Compares the total lengths of two curves or paths, quantifying how much they differ in terms of overall length.\\
\textbf{Area Difference:} Measures the difference in the area under two curves, assessing the cumulative disparity between two sets of values.\\
%
% \begin{table}[h!]
%     \centering
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{|p{3cm}|p{3cm}|p{4cm}|}
%     \hline
%     \textbf{Similarity criterion} & \textbf{Higher Value Indicates} & \textbf{Meaning of High Value} \\ \hline
%     \textbf{Euclidean Distance} & Less Similarity & Trajectories are far apart in space. \\ \hline
%     \textbf{DTW Distance} & Less Similarity & Trajectories need more non-linear alignment to match. \\ \hline
%     \textbf{Cosine Similarity} & More Similarity & Trajectories have similar orientations. \\ \hline
%     \textbf{Curve Length Difference} & Less Similarity & Trajectories differ significantly in length. \\ \hline
%     \textbf{Area Difference} & Less Similarity & Trajectories occupy different spatial regions. \\ \hline
%     \end{tabular}
%     } % End of resizebox
%     \caption{Similarity Criteria for 3D Trajectories}\label{table:similarity-criteria}
% \end{table}
\begin{table*}[ht]
\centering
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{Task}      & \textbf{Most similar DTW} & \textbf{Most similar Euclidean} & \textbf{Most similar Cosine}   & \textbf{Most similar Area diff} \\ \hline
sunface     & pic\_up    & pic\_up    & paint\_front & pic\_up       \\ \hline
shampoo     & sunface    & pic\_up    & mic          & paint\_front  \\ \hline
mic         & sunface    & pic\_up    & shampoo      & pic\_up       \\ \hline
medical     & pic\_up    & pic\_up    & washcloth    & pic\_up       \\ \hline
washcloth   & pic\_up    & pic\_up    & blowDry      & pic\_up       \\ \hline
blowDry     & sunface    & pic\_up    & washcloth    & pic\_up       \\ \hline
neut        & sunface    & pic\_up    & paint\_up    & pic\_up       \\ \hline
paint\_up   & sunface    & pic\_up    & shampoo      & pic\_up       \\ \hline
paint\_front& pic\_up    & pic\_up    & medical      & pic\_up       \\ \hline
win         & nail       & pic\_up    & shampoo      & pic\_up       \\ \hline
pic\_front  & nail       & nail       & mic          & pic\_up       \\ \hline
pic\_up     & nail       & nail       & pic\_front   & paint\_front  \\ \hline
nail        & pic\_up    & pic\_up    & neut         & pic\_up       \\ \hline
\end{tabular}
\caption{Comparison of various tasks based on different metrics.}
\end{table*}

\paragraph{Between participants.} Figure \ref{fig:Participants}, illustrates the average trajectory between participants. \textcolor{red}{similarity metrics extracted, need to fill in}
\paragraph{Between primary tasks.} Figure \ref{fig:combined_images}. 
The difference between the tasks is interesting, "hammering nail" is the furthest from the body. 
%
"balancing picture frame above head) has the highest pick point, and is [] centimeters higher than the second task.
%
"Applying sunscreen" is the closest to the user body. 
%
\textcolor{red}{similarity metrics extracted, need to fill in}
\paragraph{Hand-in vs. take-away} Figure \ref{fig:hand_in vs take_away}. "Hand-in" where robot is giving the object to the user, are happening farther from the user ([] centimeters) compared to "taking away" from the user. 
%
"hand-in"s also happen higher than the "take-away"s by average of [] centimeters.
\textcolor{red}{similarity metrics extracted, need to fill in}
\paragraph{Primary task range of motion.} Figure \ref{fig:prime_range}. 
%
In the primary tasks with shorter range of user's motion, the robot trajectory is closer to the user's body compared to the other 2 types. 
%
The trajectory in this case goes higher as weill (by average of [] centimeters)
%
Interestingly the robot trajectory for medium range of motion is happening farther from the user's body by and offset of average [] centimeters.
\textcolor{red}{similarity metrics extracted, need to fill in}
\paragraph{Primary task height.} Figure \ref{fig:prime_height}
%
The robot trajectories relative to the above the head level tasks are happening closer to the user's body (by an offset of average [] centimeters), as well as going higher (obviously!) by average of [] centimeters.
\textcolor{red}{similarity metrics extracted, need to fill in}
\paragraph{Primary task distance from user.} Figure \ref{fig:prime_distance}
\textcolor{red}{similarity metrics extracted, need to fill in}


%\paragraph{Trajectories.}
\subsection{Regions of Transfer (RoTs)}

% \begin{figure}
%     \centering
%     \includegraphics[width=\linewidth]{Source/Source_files/Figures/RoT/RoT.png}
%     \caption{Regions of transfer with directions of transfer}
%     \label{fig:enter-label}
% \end{figure}
%\paragraph{Distribution of dataset} Find out what is the distribution of our dataset (Gaussian, Exponential, Bernouli or etc.). This is crucial for the evaluation step of the generated motion, and computing the likelihood of the generated motion coming from the dataset distribution.
%\subsubsection{motion style}
\paragraph{Velocity pattern and profile trajectory}
\paragraph{Peripersonal space heat map}

%The GenAI-move dataset is composed of annotated MoCap data of participant couples mimicking the behaviour of a user wearing a hip mounted WRL. 
%
%One participant is mimicking the user who is in the first place performing a primary task, while the other participant is emulating the WRL and performing the handover task (robotic task) in collaboration with the user. 
%
%\begin{itemize}
%    \item In our setup comfort of the user matters rather than the comfort of the participant playing the WRL's role
%    \item In order to ensure that this is satisfied we make a 7-point Likert scale rating after each interaction
%\end{itemize}
%
%The recording is done in a markerless MoCap setup with 60 cameras
%


==> Source_files/Chapters/Method.tex <==
\section{Method}
\textcolor{red}{\textit{Under construction!...}}\\
In this chapter, we present the methodology and architecture of our pipeline for predicting human-robot interaction sequences and discuss our generative controller for the WRL with human-like behavior. The core of our approach is a transformer-based generative model, designed to capture the complex dynamic dependencies inherent in these interactions. 


\subsection{Model Architecture}

The transformer model employed in this study is designed to effectively model the temporal and spatial dependencies in human-robot interactions. The architecture consists of several key components: the embedding layer, positional encoding, encoder, decoder, and output layer. 

The \textbf{embedding layer} transforms input sequences into continuous vectors, which serve as the model's primary input. To retain the temporal order of the sequence, \textbf{positional encodings} are added to the embeddings, providing the model with information about the position of each element in the sequence.

The \textbf{encoder} utilizes a multi-head self-attention mechanism to weigh the importance of different time steps within the sequence, allowing the model to capture long-range dependencies. Following the attention mechanism, a feed-forward network applies non-linear transformations to the attention outputs, enhancing the model's capacity to learn complex patterns. Mathematically, the self-attention mechanism can be defined as follows:

\begin{equation}
\text{Attention}(Q, K, V) = \text{softmax}\left(\frac{QK^T}{\sqrt{d_k}}\right)V
\end{equation}

where \( Q \), \( K \), and \( V \) represent the query, key, and value matrices, respectively, and \( d_k \) is the dimension of the key vectors.

The \textbf{decoder} includes cross-attention layers that align the encoded input sequence with the target sequence, ensuring coherent predictions. The decoder also contains self-attention and feed-forward layers similar to those in the encoder, allowing it to focus on relevant parts of the input and previously generated outputs. The final \textbf{output layer} maps the decoder's output to the predicted positional and action information for the next time step.

The architecture integrates multiple specialized attention mechanisms to handle the complexity of human-robot interactions:

\begin{itemize}
  \item \textbf{Human-Robot Attention (H. R. Attn.)}: This mechanism focuses on the interaction between human and robot actions, ensuring that the model captures the dynamics of their interactions.
  \item \textbf{Human-Object Attention (H. O. Attn.)}: This mechanism captures interactions between the human and objects in the environment, which is crucial for understanding how humans manipulate objects during interactions.
  \item \textbf{Robot-Object Attention (R. O. Attn.)}: Similar to Human-Object Attention, this mechanism focuses on the robot's interactions with objects, aiding the model in learning how robots manipulate objects in response to human actions.
  \item \textbf{Temporal Attention}: This mechanism addresses the temporal progression within the sequences, allowing the model to focus on relevant time steps and capture temporal dependencies.
  \item \textbf{Spatial Attention}: This mechanism focuses on spatial relationships within the sequences, helping the model understand the spatial context of interactions.
  \item \textbf{Self Attention}: A standard transformer mechanism that allows each element of the input sequence to attend to all other elements, capturing dependencies within the sequence.
  \item \textbf{Cross Attention}: This mechanism enables the decoder to attend to the encoder's output, aligning the input and target sequences to ensure coherent predictions.
\end{itemize}

The generative process of our model can be described using a Markov chain. The model predicts the next state \( S_{t+1} \) given the current state \( S_t \) and the previous states \( S_{t-k}, \ldots, S_t \). This process can be mathematically defined as:

\begin{equation}
P(S_{t+1} | S_t, S_{t-1}, \ldots, S_{t-k}) = \text{Decoder}(\text{Encoder}(S_t, S_{t-1}, \ldots, S_{t-k}))
\end{equation}

where the encoder processes the sequence of states to capture relevant information and dependencies, and the decoder uses this encoded information to generate the prediction for the next state. The overall model aims to maximize the likelihood of the observed sequence of states, formulated as:

\begin{equation}
\mathcal{L} = \sum_{t=1}^{T} \log P(S_t | S_{t-1}, \ldots, S_{t-k})
\end{equation}



==> Source_files/Chapters/Tasks/Preliminaries.tex <==
\subsection{Preliminaries \textcolor{red}{think of a better title}}
% \paragraph{\textbf{Motion Representation.}} We define human motion as a time series data of sequential human body poses with length $T$. 
% %
% Because of our main focus on the user's body limbs' motions, rather than the whole body motion with respect to the environment, we remove the root translation and the facing direction of the user's body from our training dataset. 
% %
% We define the human body pose using the joints positions ($j_p$) and joints rotations ($j_r$). 
% %
% Similar to Motion VAE \cite{MVAE}, joint positions ($j_p \in \mathbb{R}^3$) are represented in the bodies' root space (the hips joint). 
% %
% For a continuous representation, the joints' local rotations with respect to their parent joints are represented in 6D ($j_r \in \mathbb{R}^6$) \cite{6d_continuous_representation}. 
% %
% The human pose at timestep t is a tuple of joint positions and local rotations $h^t = [j_p^t, j_r^t]$. \\
% %
% The human motion between time step $t_1$ and $t_2$ then is defined as the sequence of poses between $t_1$ and $t_2$: \\
% %
% $h^{[t_1:t_2]} = [h^{t_1}:h^{t_2}]$
% %
% Similarly, we define the robot's pose $r^t = [EE_p^t, EE_r^t]$ where $EE_p$ and $EE_r$ are the end-effector position and rotation respectively. 
% %
% The robot motion is then $r^{[t_1:t_2]} = [r^{t_1}:r^{t_2}]$. 
\paragraph{\textbf{Conditional variational autoencoders (CVAEs).}} \textbf{the math behind the CVAE I would be written here}
Variational autoencoders (VAEs) are a family of generative models that learn reconstruct their input in a probabilistic generative process. 
%
In this process the latent variable z is encoded from the prior distribution p(z) and then the 
the input x is generated by $p\theta(x\mid z)$

A generative process of the VAE is as follows: a
set of latent variable z is generated from the prior distribution $p\theta(z)$ and the data x is generated by
the generative distribution $p\theta (x\mid z)$ conditioned on z: z ~ $p\theta(z)$, x ~ $p\theta(x\mid z)$


Conditoinal VAE
% \paragraph{\textbf{Joints' Importance Extraction}}
% To get a better insight to the implicit features of our data, specially realizing the effect of every joint in the input to our models on the predicted outcome, we attempt to find out which of the individual joints is contributing more heavily (influentially) to the output. 
% %
% Among the different methods for feature importance extraction, gradient based methods are one of the well stablished approaches such as Saliency map [cit], Grad-CAM[cite] and etc.  
% %
% Saliency maps are used in visualizing the gradient of output of model with respect to the input features. 
% %
% By using the similar approach and compute the the gradient of our model's output with respect to the input joints, we are able to quantify the influence of each joint in the input on the output of the model at each time step. 
% %
% Because of the fact that gradients are naturally calculated to update the network parameters during backpropagation, they can provide a natural and effective means of tracking the effect of each of the input features. 
% %
% This is helpful enhancing our grasp of the implicit features in the dataf and provides valuable insights for feature selection or joint importance weighting. 
% %
% In our approach, we calculate the derivative of our network with respect to the inputs at each frame during the handover and for all the handover instances on the training data. 
% %
% As mentioned preveously, each joint in the input is presented with the joint's position in the user's hips coordinate and the 6D representation of the joint's local euler angles. 
% %
% For the output at each time step we calculate the magnitudes of the gradients with respect to position and rotation of each joint. 
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Source/Source_files/Figures/applications/joint_importance_pipeline.png}
    \caption{The joint importance calculation method. The derivatives of output of the trained model at each time step is calculated with respect to each joint's position and rotation, and then the average magnitude of position and rotation gradients are calculated over the dataset. The joints with the largest gradient magnitudes are reported.}
    \label{fig:importance-extraction}
\end{figure}

==> Source_files/Chapters/scratch-paper.tex <==
\section{User Study}
We conducted a user study to evaluate how participants perceive handover interactions using our data-driven approach compared to a state-of-the-art baseline~\cite{AjoudaniBiDirecontalHandover}. 

\subsection{Research Questions}
The study explored the following aspects:
\begin{itemize}
    \item \textbf{Naturalness:} How naturally do participants perceive the handover interactions? (e.g., “The interaction felt natural like human-human handovers.”)
    \item \textbf{Physical demand:} How physically demanding and comfortable are the interactions? (e.g., “The handover felt physically demanding,” “The interaction was comfortable.”)
    \item \textbf{Motion quality:} How smooth and predictable were the SRL motions? (e.g., “The motion was predictable,” “Movements were smooth and continuous.”)
    \item \textbf{Responsiveness:} Did the SRL’s responsiveness and timing meet participants’ expectations? (e.g., “The timing matched my expectations,” “The SRL reacted appropriately.”)
\end{itemize}

\subsection{Participants}
We recruited 17 participants (4 males, 13 females; ages 24–45) via the university mailing list. All participants received monetary compensation.

\subsection{Study Design}
The study followed a within-subject design where each participant performed handovers using both the baseline and data-driven methods across six primary tasks. Task order and interaction approaches were counterbalanced to mitigate order effects. The handover interactions were implemented in virtual reality (VR) due to logistical constraints and to enable naturalistic validation of the 3HANDS-trained models.

\subsubsection{Handover Approaches}
\paragraph{Baseline:}
The baseline approach uses pre-defined 3D activation regions and a Kalman filter to predict the user’s hand position. Upon activation, the SRL plans a trajectory to a target point, halting at a predefined distance, $\delta$, from the user’s hand.

\paragraph{3HANDS Data-driven Approach:}
Our approach employs a hierarchical architecture with a \textbf{"when-to"} activation model and a \textbf{"how-to"} motion generation model. The \textbf{"when-to"} model activates the SRL based on user activity, while the \textbf{"how-to"} model generates smooth, context-aware motion based on historical and current user data.

\subsection{Apparatus and Materials}
The VR environment, developed in Unity3D, was executed on a Quest Pro headset. Participants interacted with a virtual SRL mounted on their hip, and the object for handovers was a sphere at the SRL’s end-effector. Color-coded indicators distinguished the approaches: \textbf{blue} for the data-driven method and \textbf{orange} for the baseline.

\subsection{Procedure}
Participants completed a tutorial on the platform and performed 24 handover trials (12 per method). After each trial, they rated their experience on a 7-point Likert scale. The session included a semi-structured interview and lasted approximately 60 minutes.

\subsection{Data Analysis}
Likert scale responses were analyzed using Aligned Rank Transform (ART) ANOVA. Results are presented in Figure~\ref{fig:likertScaleResults}.

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Source/Source_files/Figures/userStudy/result.pdf}
    \caption{Results of the 7-point Likert scale comparing the 3HANDS (DD) and baseline (BL) approaches.}
    \label{fig:likertScaleResults}
\end{figure}

